Data-free Multi-label Image Recognition via LLM-powered Prompt Tuning

This paper proposes a novel framework for multi-label image recognition without any training data, called data-free framework, which uses knowledge of pre-trained Large Language Model (LLM) to learn prompts to adapt pretrained Vision-Language Model (VLM) like CLIP to multilabel classification. Through asking LLM by well-designed questions, we acquire comprehensive knowledge about characteristics and contexts of objects, which provides valuable text descriptions for learning prompts. Then we propose a hierarchical prompt learning method by taking the multi-label dependency into consideration, wherein a subset of category-specific prompt tokens are shared when the corresponding objects exhibit similar attributes or are more likely to co-occur. Benefiting from the remarkable alignment between visual and linguistic semantics of CLIP, the hierarchical prompts learned from text descriptions are applied to perform classification of images during inference. Our framework presents a new way to explore the synergies between multiple pre-trained models for novel category recognition. Extensive experiments on three public datasets (MS-COCO, VOC2007, and NUS-WIDE) demonstrate that our method achieves better results than the state-of-the-art methods, especially outperforming the zero-shot multi-label recognition methods by 4.7% in mAP on MS-COCO.

==> org/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> org/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> org/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> org/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/0_abstract.tex <==
\begin{abstract}
This paper introduces a data-free framework to enhance multi-label image recognition in the absence of training data. Leveraging pre-trained large language models (LLMs) and vision-language pre-trained models (VLMs) cooperatively, our method classifies images solely on a given set of object names, without any images or text descriptions for training. 
% We initiate the process by formulating a series of inquiries to LLMs to acquire comprehensive object knowledge. Subsequently, in collaboration with VLMs, we employ this knowledge to establish a graph-prompt learning paradigm that takes into consideration the relationships between objects.
Specifically, we formulate a series of inquiries into the LLMs to obtain comprehensive object knowledge.  Based on VLMs, we then employ this textual knowledge to establish a graph-prompt learning paradigm that takes into consideration the relationships between objects.
% The learned tokens of prompts may share for those categories that have similar attributes.
Thanks to the remarkable alignment between visual and linguistic semantics in VLMs, the learned graph prompts are applied to perform inferences on image inputs.
Utilizing generated textual knowledge and the relationship-aware graph prompting learning, we outperform the zero-shot multi-label image recognition by a large margin on the public benchmarks.
Our framework presents a potential direction that uncovers new objects of images that only rely on limited prior knowledge, \textit{i.e.}, object names, and a new way for further exploration of the synergies between large pre-trained models.
\end{abstract}

==> sec/1_intro.tex <==

% \section{Introduction}
% \label{sec:intro}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/intro.pdf}
%     \caption{To be replaced}
%     \label{fig:intro}
% \end{figure}
% % which typically deals with images of a diverse array of objects and scenes. 
% Multi-label image recognition aims to recognize all semantic labels present in an image.
% However, existing models struggle to adapt to the emergence of novel objects and scenes, as shown in Figure~\ref{fig:intro} (a). 
% Efforts have been made to alleviate this issue by formulating appropriate open-set problems. 
% Nonetheless, within most current open-set frameworks, the prevalent approach when confronted with newly encountered classes is to designate them as an "unknown" label, thus limiting their practical applicability.

% The pursuit of Artificial General Intelligence (AGI) has led to the development of a plethora of large-scale models known for their rich knowledge representation. Consequently, open-vocabulary tasks have gained prominence, aiming to address the issue of newly emerging categories leveraging vision-language pre-trained models, as shown in Figure~\ref{fig:intro} (b).
% A typical open-vocabulary approach conducts fine-tuning or prompt-tuning on base categories dataset, which requires training dataset, whether large or small.  A new challenge arises: how can we fine-tune the pre-trained vision-language models for multi-label image recognition when it is difficult to acquire any images?

% It is challenging to conjure an image of an entirely unfamiliar object. However, we can effectively identify the object in a picture if provided with a linguistic description. This observation inspires us to glean knowledge from language and apply them to images.
% Benefiting from the remarkable alignment of visual and linguistic semantics within the vision-language pre-trained models (VLMs), we introduce a novel framework: initially learning objects through the language modality and subsequently transferring the corresponding knowledge to the visual domain. 

% Language knowledge can be acquired through expert input or internet search engines. While relatively easier than gathering images, this process can be time-consuming and resource-intensive. Is there a more efficient alternative approach? 
% Leveraging Large Language Models (LLMs), such as OpenAI's ``ChatGPT", which stores a wealth of semantic knowledge, enables us to obtain precise responses through direct questioning, circumventing the need to sift through abundant and noisy internet pages for valuable information.
% This presents a more streamlined method for gathering language knowledge.
% Consequently, we propose a novel data-free framework:  given only the category labels without accompanying any images or texts, and we enhance multi-label image recognition by utilizing LLMs and VLMs, as shown in Figure~\ref{fig:intro} (c). 

% % Language knowledge can be collected from experts or searched by internet search engines. Though easier than images, collecting such language is time-consuming and resource-intensive. 
% % Is there a more efficient alternative way?
% % Leveraging the large language models (LLMs), like OpenAI's ``ChatGPT", which stores a wealth of semantic knowledge, we can directly get the results by asking questions instead of extracting valuable information from the abundance and noisy pages from the internet. 
% % This gives us a new way to collect language knowledge in an easier way.  
% % Hence, we propose a novel data-free framework: given only the category labels without accompanying any images or texts, we enhance multi-label image recognition by harnessing the power of LLMs and VLMs, as shown in Figure~\ref{xxx} (c). 

% % 这里有一个图，上边是train, 下边是test; a) 正常的finetune， b) 在小数据集上 prompt 大模型，c) data-free 只根据类别名字和两个大模型，得到结果。
% % Modern success in artificial intelligence relies on a large amount of data and deep learning skills. 
% % A typical process for a new task starts with collecting data, which is high-cost and time-consuming. 
% % Large pre-trained models boost most AI tasks, for their excellent capacities and generalities. 
% % % How to exploit these large pre-trained models raise most attention.
% % Although mediocre zero-shot performances have been achieved, fine-tuning or prompting tuning is needed for downstream tasks for high-performance demand. This means a training dataset is required, whether large or small. 
% % However, when no training data is accessible, could we improve the performance of the  downstream visual perception tasks compared with their zero-shot counterparts? 
% % In this paper, we improve the performance of zero-shot multi-label image recognition without accessing any image data, utilizing the pre-trained large language model and vision-language model.   
% % By only providing the category names, we first collect the information for each category from LLMs by asking specific questions. 
% % To learn different aspects of each category, we design a series of attributes for all categories, such as color, shape, texture, and so on. Then, a question like ``generate 10 sentences to describe the [attribute] of [category]" is input to the LLMs to get responses as the text descriptions of the specific category. By collecting text descriptions, we gain language knowledge about the categories based on which we conduct prompt-tuning to the text encoder of VLMs to learn task-specific prompts, demonstrating adapting the pre-trained model to downstream tasks.
% In this study, we begin with gathering the information of the provided category names. Specifically, we leverage LLMs to obtain comprehensive information for each category through targeted inquiries. To capture diverse facets of each category, we meticulously design an array of attributes describing characteristics such as color, shape, texture, and the like. Subsequently, we pose questions like ``generate 10 sentences to describe the [attribute] of [category]" to the LLMs. The responses obtained serve as textual descriptions for the specific category and are used for our subsequent prompt-tuning training of VLMs from the language aspect. Consequently,  we learn task-specific prompts, which demonstrate effectiveness in adapting the VLMs to a range of downstream tasks~\cite{xxx}.

% % For the multi-label image recognition task, the relationships of different categories are demonstrated to be effective.  As such, we learn these relationships from two aspects. The first is gathering scene information of the co-occurrence objects. We propose a new form of questions like ``generate 10 sentences to describe a scene that [category1] is [relationship] of [category2]" or ``generate 10 sentences to describe a scene of [category1], [category2], and [category3]", where [category1], [category2]  and  [category3] are in same subgroups split by their attributes. The second is we design a graph prompting learning, where we split tokens of learning prompts into three types: (1) class-shared tokens, tokens are shared over the same subgroups; (2) class-specific tokens, tokens are specific as the category varies; and (3) shared tokens, tokens are shared over all categories.  By the graph style prompts, we learn prompts considering both the task-related priors and the relationship of categories.  
% For the multi-label image recognition task, it has been demonstrated that considering the relationships between different categories can lead to more effective results. To this end, we focus on learning these relationships from two distinct perspectives. 
% The first one involves gathering scene-related information regarding the co-occurrence of objects. 
% We introduce a new form of questions, like "generate 10 sentences to describe a scene where [category1] is [relationship] of [category2]" or "generate 10 sentences to describe a scene involving [category1], [category2], and [category3]". Here, [category1], [category2], and [category3] are drawn from the same subgroup, split by their shared attributes, and [relationship] is the positional (\textit{e.g.}, above, on right) or structural (\textit{e.g.}, subpart) words. 
% Secondly, we adopt a graph-prompt learning approach, categorizing tokens of the prompts into three types: (1) class-shared tokens, which are tokens shared among categories within the same subgroups (more likely to be co-occurrence); (2) class-specific tokens, which are tokens specific to each category; and (3) shared tokens, which are tokens shared across all categories. Through this graph-style prompting, we aim to learn prompts that take into account both task-specific prior knowledge and the inter-relationships between categories.

% Thanks to the good alignment of visual and linguistic semantics of VLMs, we learn graph prompts in descriptions from LLMs and apply them to the visual inputs. By doing so, we improve the performance of multi-label image recognition by a large margin compared to the simple zero-shot approaches. 

% In conclusion, our contribution can be summarized as follows:
% (1) we propose a framework that leverages the rich knowledge stored within LLMs and VLMs to address the challenge of multi-label image recognition in scenarios where no image or text data is available. 
% (2) we design different types of questions to acquire knowledge from LLMs, both by their own characteristics and their co-occurrence.
% (3) we propose a graph-prompt learning paradigm to learn both task-specific priors, considering the co-occurrence between different categories. 
% Our framework introduces a promising avenue for uncovering new objects in images, relying solely on minimal prior knowledge, such as object names. Moreover, it paves a new way for further exploration of the synergies between large pre-trained models.


\section{Introduction}
\label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/intro.pdf}
    \caption{To be replaced}
    \label{fig:intro}
\end{figure}
% multi-label --> pre-trained model的介入-->text as image -->our method 提出-->细节 -->优势，以及和其他使用LLM方法的对比 --> contribution
% which typically deals with images of a diverse array of objects and scenes. 
Multi-label image recognition aims to recognize all semantic labels present in an image.
However, existing models struggle to adapt to the emergence of novel objects and scenes~\cite{ben2021semantic}, as shown in Figure~\ref{fig:intro} (a). 
Efforts have been made to mitigate this problem by developing appropriate unsupervised or weakly supervised methods~\cite{xxx无监督和弱监督方法}.
However, due to poor performance, there is still a long way to go before practical application.

% Efforts have been made to alleviate this issue by formulating appropriate open-set problems. 
% Nonetheless, within most current open-set frameworks, the prevalent approach when confronted with newly encountered classes is to designate them as an "unknown" label, thus limiting their practical applicability.

The pursuit of Artificial General Intelligence (AGI) has led to the development of an array of large-scale models, renowned for their extensive knowledge representation, \textit{e.g.}, CLIP~\cite{xxx}, and ChatGPT~\cite{xxx}. 
% Though good zero-shot performance is achieved, adapting these models to downstream tasks by prompt-tuning learning is still a common way for satisfied performance~\cite{xxx}, and it generally requires training data to learn prompts, as shown in Figure~\ref{fig:intro} (b).  
While these models demonstrate commendable zero-shot performance, prompt-tuning learning is still a common way achieving satisfactory results in downstream tasks~\cite{xxx}, \textit{i.e.}, multi-label image recognition. 
Nonetheless, the performance of these prompt-tuning methods may be limited when it is infeasible to obtain sufficient training data. This poses a new challenge: how can we adapt the pre-trained models for multi-label image recognition when it is infeasible to obtain any images?

% A typical prompt-tuning learning approach conducts fine-tuning or prompt-tuning on base categories dataset, which requires training dataset, whether large or small.  A new challenge arises: how can we fine-tune the pre-trained vision-language models for multi-label image recognition when it is difficult to acquire any images?
% Consequently, open-vocabulary tasks have gained prominence, aiming to address the issue of newly emerging categories leveraging vision-language pre-trained models, as shown in Figure~\ref{fig:intro} (b).
% A typical open-vocabulary approach conducts fine-tuning or prompt-tuning on base categories dataset, which requires training dataset, whether large or small.  A new challenge arises: how can we fine-tune the pre-trained vision-language models for multi-label image recognition when it is difficult to acquire any images?

It is challenging to conjure an image of an entirely unfamiliar object, but we can effectively identify the object in a picture if provided with a linguistic description. This observation inspires us to glean knowledge from language and apply it to images.
Language knowledge can be acquired through internet search engines. While relatively easier than gathering images, this process is time-consuming.
% we introduce a novel framework: initially learning knowledge through the language modality and subsequently transferring the corresponding knowledge to the visual domain. 
% Language knowledge can be acquired through expert input or internet search engines. While relatively easier than gathering images, this process can be time-consuming and resource-intensive. Is there a more efficient alternative approach? 
The Large Language Models (LLMs), such as OpenAI's ``ChatGPT", which stores a wealth of semantic knowledge, enables us to obtain precise responses through direct questioning, circumventing the need to sift through abundant and noisy internet webpages for valuable information.
% This presents a more modern method for gathering language knowledge.
And benefiting from the remarkable alignment of visual and linguistic semantics within the vision-language pre-trained models (VLMs), we propose a novel data-free framework:  given only the category labels without accompanying any images or texts, and we enhance multi-label image recognition by utilizing LLMs and VLMs cooperatively, as shown in Figure~\ref{fig:intro} (c). 
% And how to utilize these large pre-trained models comprehensively and cooperatively is still an open problem. 

% Language knowledge can be collected from experts or searched by internet search engines. Though easier than images, collecting such language is time-consuming and resource-intensive. 
% Is there a more efficient alternative way?
% Leveraging the large language models (LLMs), like OpenAI's ``ChatGPT", which stores a wealth of semantic knowledge, we can directly get the results by asking questions instead of extracting valuable information from the abundance and noisy pages from the internet. 
% This gives us a new way to collect language knowledge in an easier way.  
% Hence, we propose a novel data-free framework: given only the category labels without accompanying any images or texts, we enhance multi-label image recognition by harnessing the power of LLMs and VLMs, as shown in Figure~\ref{xxx} (c). 

% 这里有一个图，上边是train, 下边是test; a) 正常的finetune， b) 在小数据集上 prompt 大模型，c) data-free 只根据类别名字和两个大模型，得到结果。
% Modern success in artificial intelligence relies on a large amount of data and deep learning skills. 
% A typical process for a new task starts with collecting data, which is high-cost and time-consuming. 
% Large pre-trained models boost most AI tasks, for their excellent capacities and generalities. 
% % How to exploit these large pre-trained models raise most attention.
% Although mediocre zero-shot performances have been achieved, fine-tuning or prompting tuning is needed for downstream tasks for high-performance demand. This means a training dataset is required, whether large or small. 
% However, when no training data is accessible, could we improve the performance of the  downstream visual perception tasks compared with their zero-shot counterparts? 
% In this paper, we improve the performance of zero-shot multi-label image recognition without accessing any image data, utilizing the pre-trained large language model and vision-language model.   
% By only providing the category names, we first collect the information for each category from LLMs by asking specific questions. 
% To learn different aspects of each category, we design a series of attributes for all categories, such as color, shape, texture, and so on. Then, a question like ``generate 10 sentences to describe the [attribute] of [category]" is input to the LLMs to get responses as the text descriptions of the specific category. By collecting text descriptions, we gain language knowledge about the categories based on which we conduct prompt-tuning to the text encoder of VLMs to learn task-specific prompts, demonstrating adapting the pre-trained model to downstream tasks.
Specifically, we begin with gathering the information of the provided category names. More specifically, we leverage LLMs to obtain comprehensive information for each category through targeted inquiries. To capture diverse facets of each category, we meticulously design an array of attributes describing characteristics such as color, shape, texture, and so on. Subsequently, we pose questions like ``generate 10 sentences to describe the [attribute] of [category]" to the LLMs. The responses obtained serve as textual descriptions for the specific category and are used for our subsequent prompt-tuning training of VLMs from the language aspect. Consequently,  we learn task-specific prompts, which demonstrate effectiveness in adapting the VLMs to a range of downstream tasks~\cite{xxx}, and apply them to multi-label image recognition task.

% For the multi-label image recognition task, the relationships of different categories are demonstrated to be effective.  As such, we learn these relationships from two aspects. The first is gathering scene information of the co-occurrence objects. We propose a new form of questions like ``generate 10 sentences to describe a scene that [category1] is [relationship] of [category2]" or ``generate 10 sentences to describe a scene of [category1], [category2], and [category3]", where [category1], [category2]  and  [category3] are in same subgroups split by their attributes. The second is we design a graph prompting learning, where we split tokens of learning prompts into three types: (1) class-shared tokens, tokens are shared over the same subgroups; (2) class-specific tokens, tokens are specific as the category varies; and (3) shared tokens, tokens are shared over all categories.  By the graph style prompts, we learn prompts considering both the task-related priors and the relationship of categories.  
For the multi-label image recognition task, it has been demonstrated that considering the relationships between different categories can lead to more effective results. To this end, we focus on absorbing these relationships from two distinct perspectives. 
The first one involves gathering scene-related information regarding the co-occurrence of objects. 
We introduce a new form of questions, like ``generate 10 sentences to describe different scenes involving [category1] and [category2]". Here, [category1] and [category2] are drawn from the same subgroup, divided by their shared attributes.
% ``generate 10 sentences to describe a scene where [category1] is [relationship] of [category2]"
% and [relationship] is the positional (\textit{e.g.}, above, on right) or structural (\textit{e.g.}, subpart) phrases. 
Secondly, we adopt a graph-prompt learning approach, categorizing tokens of the prompts into three types: \textbf{(1)} class-shared tokens, which are tokens shared among categories within the same subgroups (more likely to be co-occurrence); \textbf{(2)} class-specific tokens, which are tokens specific to each category; and \textbf{(3)} shared tokens, which are tokens shared across all categories. Through this graph-style prompting, we aim to learn prompts that take into account both task-specific prior knowledge and the inter-relationships between categories.

Thanks to the good alignment of visual and linguistic semantics of VLMs, we learn graph-prompts in the language aspect of LLMs and can apply them to the visual inputs. By doing so, we improve the performance of multi-label image recognition by a large margin compared to the simple zero-shot approaches. 

In conclusion, our contribution can be summarized as follows:
(1) we propose a data-free framework that leverages the rich knowledge stored within LLMs and VLMs to address the challenge of multi-label image recognition in scenarios where no image or text data is available. 
(2) we design different types of questions to acquire knowledge of given object categories from LLMs, both by their own characteristics and their co-occurrence and relationships.
(3) we propose a graph-prompt learning paradigm to learn task-specific priors, considering the relationships between different objects. 
Our framework introduces a promising avenue for uncovering new objects in images, relying solely on minimal prior knowledge, such as object names. Moreover, it paves a new way for further exploration of the synergies between large pre-trained models.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
